Graph Backup: Data Efficient Backup Exploiting Markovian Transitions

The successes of deep Reinforcement Learning (RL) are limited to settings where we have a large stream of online experiences, but applying RL in the data-efficient setting with limited access to online interactions is still challenging. A key to data-efficient RL is good value estimation, but current methods in this space fail to fully utilise the structure of the trajectory data gathered from the environment. In this paper, we treat the transition data of the MDP as a graph, and define a novel backup operator, Graph Backup, which exploits this graph structure for better value estimation. Compared to multi-step backup methods such as $n$-step $Q$-Learning and TD($\lambda$), Graph Backup can perform counterfactual credit assignment and gives stable value estimates for a state regardless of which trajectory the state is sampled from. Our method, when combined with popular value-based methods, provides improved performance over one-step and multi-step methods on a suite of data-efficient RL benchmarks including MiniGrid, Minatar and Atari100K. We further analyse the reasons for this performance boost through a novel visualisation of the transition graphs of Atari games.

==> tex/checklist.tex <==
\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code is in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
    
\end{enumerate}
\end{enumerate}

==> tex/qbuffer.tex <==
\algrenewcommand\algorithmicindent{2.0em}


\begin{algorithm}[H]
\caption{DQN with GB-Q (Online Case). Blue text denotes additions of GB-Q to standard DQN.}\label{alg:backupQ}
\begin{algorithmic}[1]
\Require batch size $M$, exploration constant $\epsilon$, learning rate for tabular Q Learning $\alpha$, number steps for running Tabular Q learning $T_{\text{table}}$
target network update frequency $t_{\text{target}}$
\State Initialise online network weights $\theta$ at random
\State Observe the first state $s$
\State Initialise the set stores seen states $\mathcal{S}_{\text{seen}} \leftarrow \emptyset$
\For{$t=0$ to $T$}
    \State With probability $\epsilon$ select random action $a$, otherwise select $a=\argmax_{a'} q_{\boldsymbol \theta}(s, a')$
    \State Execute action $a$, observe reward $r$ and state $s'$
    \color{blue}
    \If{$s' \not\in \mathcal{S}_{\text{seen}}$}
    \State {Initialise the target $\hat G_{s',a'} = q_{\boldsymbol \theta'}(s',a')$ for all actions $a'$}
    \State Update seen states $\mathcal{S}_{\text{seen}} \leftarrow \mathcal{S}_{\text{seen}} \cup \{s'\}$
    \EndIf
    \color{black}
    \State Store $(s,a,r,s')$ in replay buffer
    \If{$t\mod t_{\text{target}}=0$}
        \State Update target network weights $\theta' \leftarrow \theta$
        \State \textcolor{blue}{Reinitialise targets $\hat G_{s_j,a'} = q_{\boldsymbol \theta'}(s_j,a')$ for all $a'$ and observed $s_j \in \mathcal{S}_{\text{seen}}$}
    \EndIf
    \textcolor{blue}{\For{$i=0$ to $T_{\text{table}}$}
        \State {Sample a transition $(\bar s, \bar a, \bar r, \bar s')$ from replay buffer}
        \State {Update target $\hat G^{\bar a}_{\bar s} \leftarrow \hat G^{\bar a}_{\bar s} + \alpha(\bar r + \gamma \max_{a'}\hat G_{\bar s'}^{a'} - \hat G^{\bar a}_{\bar s})$}
    \EndFor}
    \State Sample random minibatch of transitions $(s_k, a_k, r_k, s_k')$ from replay buffer
    \State Perform a gradient descent step on $|q_{\boldsymbol \theta}(s_k,a_k) - $ \textcolor{blue}{$\hat G^{s_k}_{a_k}$}$|^2$ with respect to $\theta$
    \State Update current state variable $s \leftarrow s'$
\EndFor
\end{algorithmic}
\end{algorithm}
